QuALITY: Question Answering with Long Input Texts, Yes!

To enable building and testing models on long-document comprehension, we introduce QuALITY, a multiple-choice QA dataset with context passages in English that have an average length of about 5,000 tokens, much longer than typical current models can process. Unlike in prior work with passages, our questions are written and validated by contributors who have read the entire passage, rather than relying on summaries or excerpts. In addition, only half of the questions are answerable by annotators working under tight time constraints, indicating that skimming and simple search are not enough to consistently perform well. Our baseline models perform poorly on this task (55.4%) and significantly lag behind human performance (93.5%).

==> misc.tex <==

ABSTRACT



\begin{abstract}
To enable building and testing models on long-document comprehension, 
we introduce QuALITY, a multiple-choice QA dataset with context passages in English that have an average length of about 5,000 tokens, much longer than typical current models can process. 
%To create this dataset, we hire writers to write questions that are unambiguous and answerable by attentive readers. We also encourage them to write questions that are difficult and require comprehending a large context. 
Unlike in prior work with passages,  our questions are written and validated by contributors who have read the entire passage, rather than relying on summaries or excerpts. In addition, only half of the questions are answerable by annotators working under tight time constraints, indicating that skimming and simple search aren't enough to consistently perform well. %The careful data-collection and quality-control from our validation process result in a challenging and high-quality long-document QA dataset. 
Current models perform poorly on this task (55.4\%) and significantly lag behind human performance (93.5\%). 
% Furthermore, qualitative analysis shows that over half of the questions require relatively abstract reasoning, 
% suggesting that QuALITY effectively tests for long-context reading comprehension.
\end{abstract}







INTRO





% NarrativeQA is a generation-based QA task that introduces the task of question answering for long text inputs and is extremely challenging for current models.  % This dataset uses very long contexts, with an average length of 62,743 tokens, for a generation based QA task. Full books and movie scripts are used as source texts in this dataset, but short summaries were used during data creation to make data-collection feasible. 





% However, a major challenge in creating appropriate datasets is in crowdsourcing such a time-consuming and difficult task.
% Workers need to spend a significant amount of time just reading a passage before they can begin writing questions for it, though the payment depends solely on the questions created. 
% Additionally, writing difficult yet answerable questions is a task that requires some amount of domain knowledge in literature or education, so we need to identify a population of crowdworkers with training or experience in this specific domain. 
% A related challenge comes in validating such data after it is collected. 
% The only way to validate if a question is challenging and requires having read a long passage in order to answer it correctly is for the validators to \textit{also} carefully read that passage, in its entirety. 
% Thus, the data collection process needed to create a challenging long-document QA dataset not only presents technical challenges in the collection, but is also quite time-consuming and costly.





%We therefore introduce a multiple-choice question answering dataset: QuALITY (standing for, as a slightly forced backronym, Question Answering with Long Input Text, Yes!).\footnote{\url{https://github.com/nyu-mll/quality-public}.} This dataset uses source articles that are 2k--8k tokens using spaCy tokenization,\footnote{1.5k--6k words, not counting punctuation.} and we collect high-quality multiple choice questions that are both human answerable and difficult. Specifically, we hire question writers on the freelancing platform Upwork, and we encourage them to write questions such that (1) the question is answerable and unambiguous, and an attentive reader can answer the questions correctly, (2) the question relies on evidence from multiple parts of the text instead of only a few sentences,  % \hh{How is this connected to multi-hop QA?}, % good question
% and (3) the incorrect choices look plausible given only a superficial reading of parts of the context. 

% Questions which are unambiguous and answerable by attentive readers are kept in the final dataset. Additionally, we assure challenging data by adding the constraint that a difficult question must be answerable by a human who has read the entire text, but not answerable by a human with limited time to skim the text. Questions that cannot be answered in this speed validation setting compose a difficult subset of the final dataset. 

% have not read the passage are included in QuALITY, as they will likely still be challenging for current LMs, but they are not part of the ``difficult'' subset.

% One challenge for the slow progress of long-document QA is the input length of the documents, which poses a challenge both on the modelling and on the crowdsourcing ends.  % RP: moved this paragraph to related work for now

% We use a range of models as well as extraction algorithms to ..., and we find that current models barely perform above chance. Analysis. 





% Recent work \citep{vania-etal-2021-comparing,rodriguez-etal-2021-evaluation} has shown the importance of designing datasets that can differentiate among models while having enough headroom for potential improvements. Therefore, we aim to create a long-document QA dataset where there is a significant portion of ``difficult'' examples.






WRITING




% \subsubsection {Writer Recruitment}

% % \hh{What are ideal writers you want to recruit?}

% % To achieve the goal of developing a dataset with difficult questions that require substantial understanding, 
% We need writers who have good reading comprehension skills and/or writers who have experience constructing reading comprehension questions (e.g., literature teachers who have experience writing tests for their students). 
% We hire two groups of writers on the freelancing platform Upwork (the second group two months after the first group, after we decided to increase the final size of the dataset).
% For each group, we advertise a task titled \textit{Writing college-level reading comprehension questions}. The job post is visible to all U.S. Upwork freelancers, and we specifically send out job invitations to promising freelancers who are writers or teachers, or who have college-level degrees in English, Literature, Creative Writing, Philosophy, Education, or similar fields. 

% For the first group, we received 104 applications in the span of two weeks. Of those, we selected 26 people to complete a qualification task as a paid interview. For the second group, we received 65 applications and interviewed 11.
% The interview task consists of (i) reading through detailed instructions, (ii) reading through a tutorial example passage with 10 example questions, each with an explanation of what made it a good or a bad question, and (iii) writing 10 reading comprehension questions for a new passage; regardless of whether we eventually hire them, we pay workers \$30 and estimate that this task takes 2 hours to complete. 
% Three authors (of this paper) then assess each writer's work using the following criteria: (i) whether the writer-provided correct answers are actually the correct answers, (ii) whether the questions are answerable and unambiguous, and (iii) whether more than just a few sentences of context are needed to correctly answer the questions. 
% Based on these criteria, we select the top performing 15 writers to continue on to the main task in the first group, and 7 in the second group. 

% For the 22 writers we hire after the interview, 15 have a college degree in English, literature, philosophy, creative writing, or education; 4 of these 15 writers are Ph.D. students or graduates. 11 of the 22 writers have taught high-school or college-level English or literature classes; among these 11 writers, 7 have 5+ years of teaching experience. 2 of the 22 writers mention that they write novels. 






% Bonuses on top of base rates are a feature of Upwork. Freelancers also value public project testimonials which are shown to future clients. We use these two media to incentivize workers to write high-quality questions. 

% Each writer constructs 10 questions for a given passage, completing 6-30 passages in a given round and continuing for three complete rounds.\footnote{On average, group 1 writers complete 6, 14, 30 articles for the three batches, respectively; group 2 writers complete 6, 14, 20 articles for the three batches, respectively. The writing time limits for batches 1, 2, 3 are around 1, 2, 3 weeks, respectively. Validation for any batch takes less than a week.} 
% Each round is followed by feedback about how many questions validators decide are difficult and well-written, allowing writers to improve for the next round.
% Writers earn \$12.50 per passage 
% and receive a bonus of \$1.20 for each question that meets the following criteria: (i) the majority of validators agree with the writer's original label, (ii) a majority of validators rated the question as answerable and unambiguous, and (iii) the majority of validators answered the question \textit{incorrectly} in the speed validation task (\S\ref{sec:speed-val}).
% On average, writers receive bonuses on 4.2 questions per passage, resulting in average earnings of \$17.54 per passage. Based on writer self-reports, the median time to complete one writing task is about 50 minutes, for an effective rate of \$21.05/hr. {Upwork charges fees on the workers' end. We account for this by adding an extra 20\% to their pay, bringing our final cost to \$2.10 per question.} 

% Besides using the monetary bonus as an incentive for writing answerable, unambiguous, and difficult questions, we also instruct writers that their questions should use the entire context. Throughout the course of data collection, we provide writers with detailed feedback based on validations (detailed in \S \ref{sec:untimed_val}) and this feedback includes information about how much of the passage needed to be read in order to answer the question. We monitor the proportion of questions that require more than a few paragraphs of context to answer correctly; if this rate significantly lags behind other writers, we inform the writers that their work is falling below expectations and ask them to be more careful with this issue in the next round. 
% % 
% We also encourage writers to write difficult distractors, and the feedback we provide also contains what annotators think is the most difficult distractor for each question (\S \ref{sec:untimed_val}). 

% If writers have fewer than 40\% of questions meet the above three bonus criteria \emph{and} fewer than 75\% of questions meet criteria (i) and (ii), we exclude them from future writing rounds: One writer was excluded after batch 1, and one writer was excluded after batch 2, for this reason. We also exclude two writers who missed deadlines by significant margins. Two other writers voluntarily left the project before finishing all three batches.






ANNOTATOR RECRUITMENT


% \subsubsection{Annotator Recruitment}
% \label{sec:annotator-recruitment}

% % qualification task
% We recruit annotators via Amazon Mechanical Turk (MTurk).
% We use a qualification task to identify annotators with good reading comprehension skills.
% This task is open to all workers with more than 1000 tasks (HITs) accepted and a HIT accept rate of at least 98\%.
% We pay \$5 for completing the qualification task, plus a \$5 bonus for passing it.
% The task consists of a $\sim$3000-word passage with 10 multiple choice questions written or reviewed by the authors, each with a series of evaluation questions asking about the quality of that question.
% Of the 10 questions, 2 are intentionally ambiguous\footnote{We later found that one question was \textit{unintentionally} ambiguous; we do not use this question in assessing whether workers pass the qualification.} in order to test if workers can accurately identify poorer quality questions.

% % criteria to get the qualification
% In order to pass the qualification, workers need to (i) get at least 6/7 or 7/8 of the unambiguous questions correct, (ii) correctly identify at least one of the two ambiguous questions as ambiguous/unanswerable, and (iii) correctly identify at least half of the unambiguous questions as unambiguous.
% A total of 148 crowdworkers completed the task, and 45 of them passed (30.4\%).
% All workers who pass the qualification are invited to complete tasks as part of both the speed validation and the untimed validation.









SPEED ANNOTATION




% \paragraph{Catch Questions}
% We expect accuracy in the speeded task to be fairly low, so we construct catch questions to ensure that workers are not randomly guessing without attempting to find the correct answer.
% These trials are written by the authors and are designed to be answerable with only 45 seconds of access to the passage.
% % For example, catch questions may ask who spoke a certain quote, giving the exact text that could be searched to find the correct part of the passage.
% For example, a catch question may ask who spoke a quote, like ``Who said `You're a wizard Harry!'?'', where a single ctrl+F search of the quote gives the annotator the answer. Another catch question may have four options, three of which are clearly improbable. 
% We do not validate the catch questions for correctness in the untimed validation, and so we do not include them in the final dataset, but we release them as a supplemental file for reproducibility.









% \paragraph{Annotator Performance}
% Individual annotators consistently scored well above the chance rate of 25\% on the catch questions.
% In all cases where an annotator's accuracy fell below 50\% in a round, they were removed from future rounds.\footnote{Two annotators fell below this threshold, though in that round they had also performed below threshold in the untimed validation. No annotators needed to be removed \textit{solely} based on performance in the speed validation task.}
% Average overall accuracy on the catch questions was 83.8\%, indicating that most workers were able to develop a strategy for finding a correct answer when it could be found.

% Accuracy on the questions written by Upwork writers was 48.2\% overall, but annotators got better at this task over time, likely by developing new strategies to search for answers.
% Average accuracy was 39.5\% in the first round, rising to 58.4\% in the final round of data collection.
% When the majority of annotators (at least 3/5) are able to answer questions correctly in this setting, we exclude that question from the difficult subset. %interpret this as the question being too easy.
% %The reason for this easiness is most likely either due to the answer being searchable in the text or the distractor options being too improbable.










UNTIMED ANNOTATION


% \paragraph{Annotator Performance}
% % average performance
% When a label can be assigned through majority vote of just the annotators, individual annotator agreement with the majority vote answer is 89.7\% for all items identified as answerable and unambiguous, and 91.2\% for across all examples that make it into the clean version of the dataset after taking the original writer's label into consideration.






% % criteria to keep the qualification
% Throughout the course of the study, workers need to maintain at least 75\% accuracy each round to maintain the qualification and continue to the next round.\footnote{In a few cases, we identify passages that are themselves ambiguous or especially difficult. In these cases, we do not use those passages in computing by-round accuracy for the annotators.}
% % number of annotators at each round
% We exclude a total of 11 workers throughout the course of data collection for low accuracy, most of them after the first or second round.

% \paragraph{Data Reannotation}
% % automatic reannotation
% During each untimed validation round, we keep track of the rate at which each worker agrees with the original writers' labels for each question in order to quickly identify cases where either (i) a worker has misunderstood the passage, or (ii) a worker is putting insufficient effort towards the task.
% For any tasks where the individual annotator disagrees with the writer's labels on at least 40\% of questions, we automatically re-post that passage for reannotation and replace the data, with the assumption that the annotator may have misunderstood something crucial in the passage.\footnote{We identified 10 passages that, after multiple rounds of reannotation, were not passing this threshold. This may be due to one of the writers misunderstanding the passage and thereby creating several ambiguous questions, so for these 10 passage we chose to include \textit{all} annotations collected.} %, there were an insufficient number of annotations that passed this threshold after at least one set of reannotations. In all 10 cases, the average score of all annotations collected was at or below 65\%, indicating that it is likely the passage has several low-quality or ambiguous questions, and thus further reannotations will not solve the issue. When this happens, we include all annotations collected on the passage, as our original assumption that the annotators misunderstood the passage was likely incorrect.}
% % maj. vote based reannoation
% After all the annotations are complete, we calculate the gold label answer via majority vote of annotators plus the original writer's label, and assess individual annotator accuracy.
% %For any examples where no label accounts for more than 50\% of the labels, we exclude that item from the dataset (\todo{percent of all examples this happened to}.
% If any worker is excluded in a round for low accuracy (i.e., below 75\% accuracy), we discard all of their responses from that round, reannotate and replace their data, and re-calculate the gold label and accuracy scores.







ANALYSIS


% We additionally plot a normalized distribution of lexical overlap for all the correct and incorrect options (instead of considering the maximum across the three incorrect options for each question) in Figure~\ref{fig:lexical_overlap_avg}. Both the distributions are close, thus giving a similar conclusion that models would not be able to exploit the lexical overlap heuristic.









MODELING


% , while the Longformer Encoder-Decoder (LED) models support up to 16,384 encoder input tokens.




% \begin{table}[h]
% \setlength{\tabcolsep}{3.0pt}
% \centering
% \small
% \begin{tabular}{lccc}
%     \toprule
%      & correct & incorrect & total \\
%     \midrule
%     difficult & 505 & 560 & 1065 \\
%     non-difficult & 613 & 408 & 1021 \\
%     total & 1118 & 968 & 2086 \\ 
%     \bottomrule
% \end{tabular}
% \caption{Result of DeBERTa-large (using question-based extraction through DPR) for difficult vs. non-difficult questions, on development set.
% }
% \label{tab:machine-human-difficulty}
% \end{table}

% For instance, Table~\ref{tab:machine-human-difficulty} shows that RoBERTa-large using DPR extraction (the best-performing non-cheating model) answers 47.4\% of the QuALITY-\textsc{hard} questions correctly, and the model answers 60.0\% of the QuALITY-\textsc{easy} (i.e., the questions in QuALITY that are not in the hard subset) questions correctly. 






% Given the machine-human performance gap, we test if extracting more appropriate sentences is a promising research direction that would improve model performance on QuALITY. We thus conduct experiments using oracle-answer-based extraction strategies. 


% Results that rely on oracle-answer-based extraction can be found in Appendix \ref{app:results}. At test time, we assume the existence of oracle answers, so this strategy is unrealistic, and should not be compared to results in \ref{tab:main-results}. We see that the performance improves significantly (78.3\%), but is still below human performance by 15 points. 








RELATED

% \paragraph{Data.}

% \begin{itemize}
%     \item SQuAD v1.1 \citep{rajpurkar-etal-2016-squad}
%     \item SQuAD v2.0 \citep{rajpurkar-etal-2018-know}
%     \item TriviaQA \citep{joshi-etal-2017-triviaqa}
%     \item NarrativeQA \citep{kocisky-etal-2018-narrativeqa}
%     \item Wikihop \citep{welbl-etal-2018-constructing}
%     \item HotpotQA\citep{yang-etal-2018-hotpotqa}
%     \item ELI5 \citep{fan-etal-2019-eli5}
%     \item NewsQuizQA \citep{lelkes2021quiz}
%     \item \citet{krishna-etal-2021-hurdles}
% \end{itemize}


% \paragraph{Modeling.}

% \begin{itemize}
%     \item Longformer \citep{beltagy2020longformer}
%     \item T5 \citep{raffel2020t5}
%     \item UnifiedQA \citep{khashabi-etal-2020-unifiedqa}
%     \item Extraction: DPR \citep{karpukhin-etal-2020-dense}
% \end{itemize}



\section{Related Work}
\label{sec:related}

% There have been numerous QA datasets created in the last few years, and they can be roughly categorized in the following categories:

\citet{rogers2021qa} surveys the QA dataset explosion of recent years and the many formats and types of QA datasets. The QA datasets closest to our work either have long contexts or require consolidating information from multiple parts of the source text through multi-hop reasoning.

% There have been numerous QA datasets with contexts longer than SQuAD \citep{rajpurkar-etal-2016-squad, rajpurkar-etal-2018-know} in the past few years. 

% this paragraph talks about extractive qa
TriviaQA \citep{joshi-etal-2017-triviaqa} and SearchQA \citep{Dunn2017SearchQAAN} contain questions with more than one document as the context, but since the supporting documents are collected after writing the question-answer pairs, most questions can be answered after retrieving a short context. HotpotQA \citep{yang-etal-2018-hotpotqa}, QAngaroo \citep{welbl-etal-2018-constructing} and ComplexWebQuestions \citep{talmor-berant-2018-web} were constructed to have more challenging questions which require multi-hop reasoning across multiple paragraphs. However, there has been recent work \citep{jiang-bansal-2019-avoiding, min-etal-2019-compositional} showing that these datasets contain reasoning shortcuts and a large fraction of the questions can be answered with single-hop reasoning. %Additionally, by the very nature of how these datasets were created, models which first extract a small set of relevant paragraphs which are then fed into a reading comprehension model can perform very well. In contrast, similar baselines perform much worse on our dataset (\S\ref{sec:modeling}) since a lot of the questions require a thorough understanding of the complete article.

% this paragraph on abstractive qa
% Abstractive QA datasets have also been proposed. MS MARCO \citep{Campos2016MSMA}, CoQA \cite{reddy-etal-2019-coqa}, NarrativeQA \citep{kocisky-etal-2018-narrativeqa} and ELI5 \cite{fan-etal-2019-eli5} contain questions with human-generated answers and the evaluation of model answers usually requires automatic metrics such as BLEU, ROUGE etc. which have their own problems \citep{novikova-etal-2017-need, krishna-etal-2021-hurdles}. 

NarrativeQA \citep{kocisky-etal-2018-narrativeqa} is the most similar work to ours. NarrativeQA uses entire Gutenberg books and film scripts as contexts, with an average length of 60k tokens. The authors creatively make the data-collection task tractable by using Wikipedia summaries for the books as context when crowdsourcing questions. %While the task is very challenging for existing models, part of the challenge is that the contexts are so large that they do not fit within the memory of current models, like Transformer based models. Furthermore, human performance can't be readily established on the dataset since the task would require asking annotators to read full length books before answering the questions. %. 
Unlike QuALITY, NarrativeQA is a free-form generation-based task. 
%This comes with the challenge of fairly measuring model accuracy since it has been found that standard metrics for generation like BLUE \citep{papineni-etal-2002-bleu}, ROUGE \citep{lin-2004-rouge}, and BERTScore \citep{Zhang2020BERTScore} may not accurately measure quality of model generations \citep{wang-etal-2020-asking, durmus-etal-2020-feqa}.
And while there are many existing multiple-choice QA datasets  \citep{richardson-etal-2013-mctest, Hill2016TheGP, lai-etal-2017-race, Bajgar2016EmbracingDA, huang-etal-2019-cosmos}, these datasets use much shorter context passages (<500 tokens) than our dataset.

One of the primary challenges of building a long-document QA dataset like QuALITY or NarrativeQA is building a tractable crowdsourcing pipeline that enables collecting high-quality examples. \citet{roit-etal-2020-controlled} collect a challenging QA-SRL dataset by carefully hiring and training crowdworkers, with a strict qualification followed by 2 hours of training that includes giving workers extensive feedback. \citet{nangia-etal-2021-ingredients} compare crowdsourcing methods for collecting high-quality QA data and find that a long training process with iterative feedback and qualifications is an effective crowdsourcing strategy.  

% On a different note, one challenge for the slow progress of long-document QA is the input length of the documents, which poses a challenge both on the modeling and on the crowdsourcing ends. State-of-the-art language understanding models usually depend on transformers \citep{vaswani2017transformer}, but they are only recently able to accept long inputs \citep{beltagy2020longformer,zaheer2020bigbird}. Even so, these models' reasoning ability even on simple synthetic tasks is far from perfect \citep{tay2021long}. Recent extraction-based methods \citep{karpukhin-etal-2020-dense} are able to greatly boost the performance on open-domain QA tasks. While we have open-domain QA datasets, the challenge in those tasks is often finding the short excerpt that answers the questions at hand. While long-document QA requires reading the whole context and understanding it as a whole to correctly answer questions.



\section{Conclusion}
\label{sec:conclusion}

We introduce the long-document QA dataset QuALITY. This dataset was crowdsourced and validated by humans to ensure that the questions are answerable, unambiguous, and challenging. The QuALITY-\textsc{hard} subset, comprising half the dataset, consists of questions that are unanswerable by annotators working under tight time constraints, helping ensure that skimming and simple search don't yield high performance. %The examples included in QuALITY consistently ask questions that require consolidating information across the long passage

We find that current models significantly lag behind human performance on QuALITY, with a 38.1 percentage point gap between human annotators and the best performing model. The gap is even wider on QuALITY-\textsc{hard}, at 42.3 points.
We hope that research that aims at this gap will contribute to expanding the scope of texts on which effective NLU systems can be applied.
% Long-document understanding is clearly far from solved and bridging this gap on QuALITY may require skill sets that cannot be simply brute-forced by large-scale language models. For example, solving QuALITY may require machines to model changing relationships between characters and entities, and more effectively summarize long passages. 











APPENDIX 

%\paragraph{Findings}
%Despite questions using `what' being the most frequent in the question-types analysis (see Table \ref{tab:questiontypes}), very few of the questions in QuALITY depend on reasoning about objects or entities.
%Rather, most of these `what' questions are asking about the description of a person or situation, or they are asking for an interpretation from the reader.



==> tables_figures/tab_writer_stats.tex <==

\begin{table}[h]
\setlength{\tabcolsep}{3.0pt}
\centering
\small
\begin{tabular}{ccc}
    \toprule
    Batch & \makecell[c]{\# Writers} & \makecell[c]{\# Articles \\ Per Writer} \\
    \midrule
    g1b1 & 15 & 6 \\
    g1b2 & 14 & 12 \\
    g1b3 & 9 & 30 \\
    g2b1 & 7 & 6 \\
    g2b2 & 6 & 14 \\
    g2b3 & 7 & 20 \\
    \bottomrule
\end{tabular}
\caption{Writer and article stats for each batch. Note (a): One writer had an emergency after g1b2, so this writer did not work on g1b3, but returned for g2b3. Note (b): each writer wrote 14 articles for g1b2, two of which are Switchboard conversational texts. But we dropped them from the final data and all analysis due to reasons in Section~[ref]. \pang{Discuss emergencies.}
}
\label{tab:writer-stats}
\end{table}

